Multi-channel, multi-template event reconstruction for SuperCDMS data using machine learning

SuperCDMS SNOLAB uses kilogram-scale germanium and silicon detectors to search for dark matter. Each detector has Transition Edge Sensors (TESs) patterned on the top and bottom faces of a large crystal substrate, with the TESs electrically grouped into six phonon readout channels per face. Noise correlations are expected among a detector's readout channels, in part because the channels and their readout electronics are located in close proximity to one another. Moreover, owing to the large size of the detectors, energy deposits can produce vastly different phonon propagation patterns depending on their location in the substrate, resulting in a strong position dependence in the readout-channel pulse shapes. Both of these effects can degrade the energy resolution and consequently diminish the dark matter search sensitivity of the experiment if not accounted for properly. We present a new algorithm for pulse reconstruction, mathematically formulated to take into account correlated noise and pulse shape variations. This new algorithm fits N readout channels with a superposition of M pulse templates simultaneously - hence termed the N$\times$M filter. We describe a method to derive the pulse templates using principal component analysis (PCA) and to extract energy and position information using a gradient boosted decision tree (GBDT). We show that these new N$\times$M and GBDT analysis tools can reduce the impact from correlated noise sources while improving the reconstructed energy resolution for simulated mono-energetic events by more than a factor of three and for the 71Ge K-shell electron-capture peak recoils measured in a previous version of SuperCDMS called CDMSlite to $<$ 50 eV from the previously published value of $\sim$100 eV. These results lay the groundwork for position reconstruction in SuperCDMS with the N$\times$M outputs.

==> authorlist.tex <==
\author{M.F.~Albakry} %\affiliation{Department of Physics \& Astronomy, University of British Columbia, Vancouver, BC V6T 1Z1, Canada}%\affiliation{TRIUMF, Vancouver, BC V6T 2A3, Canada}
\author{I.~Alkhatib} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{D.~Alonso-González} %\affiliation{Departamento de F\'{\i}sica Te\'orica, Universidad Aut\'onoma de Madrid, 28049 Madrid, Spain%\affiliation{Instituto de F\'{\i}sica Te\'orica UAM-CSIC, Campus de Cantoblanco, 28049 Madrid, Spain}
\author{D.W.P.~Amaral} %\affiliation{Department of Physics, Durham University, Durham DH1 3LE, UK}
\author{J.~Anczarski} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{T.~Aralis} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{T.~Aramaki} %\affiliation{Department of Physics, Northeastern University, 360 Huntington Avenue, Boston, MA 02115, USA}
\author{I.~Ataee~Langroudy} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{C.~Bathurst} %\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{R.~Bhattacharyya} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{A.J.~Biffl} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{P.L.~Brink} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{M.~Buchanan} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{R.~Bunker} %\affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\author{R.~Calkins} %\affiliation{Department of Physics, Southern Methodist University, Dallas, TX 75275, USA}
\author{R.A.~Cameron} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{C.~Cartaro} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{D.G.~Cerde\~no} %\affiliation{Departamento de F\'{\i}sica Te\'orica, Universidad Aut\'onoma de Madrid, 28049 Madrid, Spain%\affiliation{Instituto de F\'{\i}sica Te\'orica UAM-CSIC, Campus de Cantoblanco, 28049 Madrid, Spain}
\author{Y.-Y.~Chang} %\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\author{M.~Chaudhuri} %\affiliation{National Institute of Science Education and Research, An OCC of Homi Bhabha National Institute, Jatni 752050, India}
\author{J.-H.~Chen} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{R.~Chen} %\affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{N.~Chott} %\affiliation{Department of Physics, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\author{J.~Cooley} %\affiliation{SNOLAB, Creighton Mine \#9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada}%\affiliation{Department of Physics, Southern Methodist University, Dallas, TX 75275, USA}
\author{H.~Coombes} %\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{P.~Cushman} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{R.~Cyna} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{S.~Das} %\affiliation{National Institute of Science Education and Research, An OCC of Homi Bhabha National Institute, Jatni 752050, India}
\author{S.~Dharani} %\affiliation{Department of Physics \& Astronomy, University of British Columbia, Vancouver, BC V6T 1Z1, Canada}
\author{M.L.~di~Vacri} %\affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\author{M.D.~Diamond} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{M.~Elwan} %\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{S.~Fallows} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{E.~Fascione} %\affiliation{Department of Physics, Queen's University, Kingston, ON K7L 3N6, Canada}%\affiliation{TRIUMF, Vancouver, BC V6T 2A3, Canada}
\author{E.~Figueroa-Feliciano} %\affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{S.L.~Franzen} %\affiliation{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\author{A.~Gevorgian} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}
\author{M.~Ghaith} %\affiliation{College of Natural and Health Sciences, Zayed University, Dubai, 19282, United Arab Emirates}
\author{G.~Godden} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{J.~Golatkar} %\affiliation{Kirchhoff-Institut f{\"u}r Physik, Universit{\"a}t Heidelberg, 69117 Heidelberg, Germany}
\author{S.R.~Golwala} %\affiliation{Division of Physics, Mathematics, \& Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\author{R.~Gualtieri} %\affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{J.~Hall} %\affiliation{SNOLAB, Creighton Mine \#9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada}%\affiliation{Laurentian University, Department of Physics, 935 Ramsey Lake Road, Sudbury, Ontario P3E 2C6, Canada}
\author{S.A.S.~Harms} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{C.~Hays} %\affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{B.A.~Hines} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}
\author{Z.~Hong} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{L.~Hsu} %\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\author{M.E.~Huber} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}%\affiliation{Department of Electrical Engineering, University of Colorado Denver, Denver, CO 80217, USA}
\author{V.~Iyer} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{V.K.S.~Kashyap} %\affiliation{National Institute of Science Education and Research, An OCC of Homi Bhabha National Institute, Jatni 752050, India}
\author{S.T.D.~Keller} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{M.H.~Kelsey} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{K.T.~Kennard} %\affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{Z.~Kromer} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}
\author{A.~Kubik} %\affiliation{SNOLAB, Creighton Mine \#9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada}
\author{N.A.~Kurinsky} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{M.~Lee} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{J.~Leyva} %\affiliation{Department of Physics, Northeastern University, 360 Huntington Avenue, Boston, MA 02115, USA}
\author{B.~Lichtenberg} %\affiliation{Kirchhoff-Institut f{\"u}r Physik, Universit{\"a}t Heidelberg, 69117 Heidelberg, Germany}
\author{J.~Liu} %\affiliation{Department of Physics, Southern Methodist University, Dallas, TX 75275, USA}
\author{Y.~Liu} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{E.~Lopez~Asamar} %\affiliation{Departamento de F\'{\i}sica Te\'orica, Universidad Aut\'onoma de Madrid, 28049 Madrid, Spain%\affiliation{Instituto de F\'{\i}sica Te\'orica UAM-CSIC, Campus de Cantoblanco, 28049 Madrid, Spain}
\author{P.~Lukens} %\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}
\author{R.~López~Noé} %\affiliation{Departamento de F\'{\i}sica Te\'orica, Universidad Aut\'onoma de Madrid, 28049 Madrid, Spain
\author{D.B.~MacFarlane} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{R.~Mahapatra} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{J.S.~Mammo} %\affiliation{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\author{A.J.~Mayer} %\affiliation{TRIUMF, Vancouver, BC V6T 2A3, Canada}
\author{P.C.~Mcnamara} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{\'E.~Michaud} %\affiliation{D\'epartement de Physique, Universit\'e de Montr\'eal, Montr\'eal, Québec H3C 3J7, Canada}
\author{E.~Michielin} %\affiliation{Institute for Astroparticle Physics (IAP), Karlsruhe Institute of Technology (KIT), 76344 Eggenstein-Leopoldshafen, Germany}
\author{K.~Mickelson} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}
\author{N.~Mirabolfathi} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{M.~Mirzakhani} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{B.~Mohanty} %\affiliation{National Institute of Science Education and Research, An OCC of Homi Bhabha National Institute, Jatni 752050, India}
\author{D.~Mondal} %\affiliation{National Institute of Science Education and Research, An OCC of Homi Bhabha National Institute, Jatni 752050, India}
\author{D.~Monteiro} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{J.~Nelson} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{H.~Neog} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{J.L.~Orrell} %\affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\author{M.D.~Osborne} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{S.M.~Oser} %\affiliation{Department of Physics \& Astronomy, University of British Columbia, Vancouver, BC V6T 1Z1, Canada}%\affiliation{TRIUMF, Vancouver, BC V6T 2A3, Canada}
\author{L.~Pandey} %\affiliation{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\author{S.~Pandey} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{R.~Partridge} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{P.K.~Patel} %\affiliation{Department of Physics \& Astronomy, Northwestern University, Evanston, IL 60208-3112, USA}
\author{D.S.~Pedreros} %\affiliation{D\'epartement de Physique, Universit\'e de Montr\'eal, Montr\'eal, Québec H3C 3J7, Canada}
\author{W.~Peng} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{W.L.~Perry} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{R.~Podviianiuk} %\affiliation{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\author{M.~Potts} %\affiliation{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\author{S.S.~Poudel} %\affiliation{Department of Physics, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\author{A.~Pradeep} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{M.~Pyle} %\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}%\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{W.~Rau} %\affiliation{TRIUMF, Vancouver, BC V6T 2A3, Canada}
\author{E.~Reid} %\affiliation{Department of Physics, Durham University, Durham DH1 3LE, UK}
\author{T.~Reynolds} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{M.~Rios} %\affiliation{Departamento de F\'{\i}sica Te\'orica, Universidad Aut\'onoma de Madrid, 28049 Madrid, Spain%\affiliation{Instituto de F\'{\i}sica Te\'orica UAM-CSIC, Campus de Cantoblanco, 28049 Madrid, Spain}
\author{A.~Roberts} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}
\author{A.E.~Robinson} %\affiliation{D\'epartement de Physique, Universit\'e de Montr\'eal, Montr\'eal, Québec H3C 3J7, Canada}
\author{L.~Rosado~Del~Rio} %\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{J.L.~Ryan} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{T.~Saab} %\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{D.~Sadek} %\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{B.~Sadoulet} %\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}%\affiliation{Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}
\author{S.P.~Sahoo} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{I.~Saikia} %\affiliation{Department of Physics, Southern Methodist University, Dallas, TX 75275, USA}
\author{S.~Salehi} %\affiliation{Department of Physics \& Astronomy, University of British Columbia, Vancouver, BC V6T 1Z1, Canada}
\author{J.~Sander} %\affiliation{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\author{B.~Sandoval} %\affiliation{Division of Physics, Mathematics, \& Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Sattari} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{R.W.~Schnee} %\affiliation{Department of Physics, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\author{B.~Serfass} %\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\author{A.E.~Sharbaugh} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}
\author{R.S.~Shenoy} %\affiliation{Division of Physics, Mathematics, \& Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\author{A.~Simchony} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{P.~Sinervo} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{Z.J.~Smith} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{R.~Soni} %\affiliation{TRIUMF, Vancouver, BC V6T 2A3, Canada}
\author{K.~Stifter} %\affiliation{SLAC National Accelerator Laboratory/Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025, USA}
\author{J.~Street} %\affiliation{Department of Physics, South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}
\author{M.~Stukel} %\affiliation{SNOLAB, Creighton Mine \#9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada}
\author{H.~Sun} %\affiliation{Department of Physics, University of Florida, Gainesville, FL 32611, USA}
\author{E.~Tanner} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{N.~Tenpas} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{D.~Toback} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{A.N.~Villano} %\affiliation{Department of Physics, University of Colorado Denver, Denver, CO 80217, USA}
\author{J.~Viol} %\affiliation{Kirchhoff-Institut f{\"u}r Physik, Universit{\"a}t Heidelberg, 69117 Heidelberg, Germany}
\author{B.~von~Krosigk} %\affiliation{Kirchhoff-Institut f{\"u}r Physik, Universit{\"a}t Heidelberg, 69117 Heidelberg, Germany}%\affiliation{Institute for Astroparticle Physics (IAP), Karlsruhe Institute of Technology (KIT), 76344 Eggenstein-Leopoldshafen, Germany}
\author{O.~Wen} %\affiliation{Division of Physics, Mathematics, \& Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Z.~Williams} %\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, MN 55455, USA}
\author{M.J.~Wilson} %\affiliation{Department of Physics \& Astronomy, University of British Columbia, Vancouver, BC V6T 1Z1, Canada}
\author{J.~Winchell} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{S.~Yellin} %\affiliation{Department of Physics, Stanford University, Stanford, CA 94305, USA}
\author{B.A.~Young} %\affiliation{Department of Physics, Santa Clara University, Santa Clara, CA 95053, USA}
\author{B.~Zatschler} %\affiliation{SNOLAB, Creighton Mine \#9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada}%\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{S.~Zatschler} %\affiliation{SNOLAB, Creighton Mine \#9, 1039 Regional Road 24, Sudbury, ON P3Y 1N2, Canada}%\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{A.~Zaytsev} %\affiliation{Institute for Astroparticle Physics (IAP), Karlsruhe Institute of Technology (KIT), 76344 Eggenstein-Leopoldshafen, Germany}
\author{E.~Zhang} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{L.~Zheng} %\affiliation{Department of Physics and Astronomy, and the Mitchell Institute for Fundamental Physics and Astronomy, Texas A\&M University, College Station, TX 77843, USA}
\author{A.~Zuniga} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada}
\author{M.J.~Zurowski} %\affiliation{Department of Physics, University of Toronto, Toronto, ON M5S 1A7, Canada} 
